Understanding factors behind IoT privacy -- A user's perspective on RF sensors

While IoT sensors in physical spaces have provided utility and comfort in our lives, their instrumentation in private and personal spaces has led to growing concerns regarding privacy. The existing notion behind IoT privacy is that the sensors whose data can easily be understood and interpreted by humans (such as cameras) are more privacy-invasive than sensors that are not human-understandable, such as RF (radio-frequency) sensors. However, given recent advancements in machine learning, we can not only make sensitive inferences on RF data but also translate between modalities. Thus, the existing notions of privacy for IoT sensors need to be revisited. In this paper, our goal is to understand what factors affect the privacy notions of a non-expert user (someone who is not well-versed in privacy concepts). To this regard, we conduct an online study of 162 participants from the USA to find out what factors affect the privacy perception of a user regarding an RF-based device or a sensor. Our findings show that a user's perception of privacy not only depends upon the data collected by the sensor but also on the inferences that can be made on that data, familiarity with the device and its form factor as well as the control a user has over the device design and its data policies. When the data collected by the sensor is not human-interpretable, it is the inferences that can be made on the data and not the data itself that users care about when making informed decisions regarding device privacy.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> Sources/1-introduction.tex <==
\section{Introduction}\label{sec:intro}

With the recent growth in the Internet-of-Things (IoT), sensors and sensing devices have infiltrated all aspects of our daily life – in smart homes, office spaces, and public areas. The data collected by these sensors provide utility to the users whose data is being collected (e.g. fitness activity tracking), or the device owner (e.g. home security). However, the opaque data collection, storage, and processing by manufacturers and device operators has motivated a discussion on privacy - particularly, how to instrument physical spaces with sensors and what to disclose to the sensed users~\cite{naeini2017privacy, igp2015protecting, emami-naeini_ask_2020}.

Privacy discussions on \textit{invasiveness}~\cite{lee2017privacy, psychoula2018users, gochoo_device-free_2018} or \textit{sensitivity}~\cite{zhou2015information} of sensors informally allude to protecting the information representing a monitored user's actions and behaviors in the physical world. 

\noindent\textbf{Problem.} Despite several definitions of privacy (\secref{sec:terms}), recent literature in IoT sensing uses human-understandability as a proxy for privacy. A common notion of privacy invasiveness in these works is that sensors which capture data easily understood by human sensory organs (e.g. visual and audio recordings) should not be placed in physically privacy-sensitive areas (e.g. bedrooms, changing rooms, or washrooms)~\cite{taylor2010spy, schwartz2012chicago}. This notion is the premise for several recent works claiming that lower-dimensional RF sensors are more privacy-sensitive than visual sensors~\cite{singh2019radhar, billah_ble_2021, aziz_shah_privacy-preserving_2020, rahaman_tracking_2021, ashleibta_non-invasive_2021, liu_beyond_2019, zeng_multisense_2020, yin_ubiquitous_2022,feng_sitr_2020, gurbuz_american_2021, li_sitsen_2021, yang_rf-eletter_2021, wang_multi-person_2021, fan_-home_2020, saeed_multiple_2022, raeis_human_2021, avrahami_below_2018, liu_wi-psg_2021}.  

\noindent\textbf{Probable Reasoning.} Even though these works do not specify why they use human-understandability as a proxy for privacy, we suspect that this is due to the fact that a majority of users that encounter these devices are non-expert i.e. they either do not have any knowledge of various definitions of privacy or they lack the necessary background to comprehend it. They instead rely on their past experiences and first impressions to make judgements about the privacy characteristics of a device or a sensor. Hence, in this paper, our focus is on understanding how non-expert users perceive privacy when they encounter a device or a sensor and are given some basic information about the device.

Some of the works in IoT sensing domain claim that raw RF sensor data reveals less information than visual data such as camera images \cite{fan_-home_nodate, raeis_human_2021, avrahami_below_2018} due to poor interpretability by humans. In reality, raw information collected by a visual sensor is not an image but merely radiation on the individual pixel sensors, which is later translated, processed, and presented as human-understandable images~\cite{isola2011understanding}. Similarly, low-dimensional RF sensor data can be translated, abstracted, or ``imaged" into privacy-sensitive information. This begs the question:
\newline 
\textit{\textbf{RQ1a}. If we take non human-understandable data collected by a sensor and convert it into a more understandable form, will that change the user's privacy perceptions about that sensor?}


While humans cannot understand the information collected by RF sensors (e.g. EM radiation collected at the receiver generally represented in the form of IQ samples~\cite{scott2001development}), they can certainly understand the inferences that algorithms can make on that data. Importantly, advances in deep learning have enabled various inferences from RF data. These various inferences may be privacy-sensitive, such as human emotion~\cite{zhao2016emotion} and several forms of human activity recognition~\cite{singh2019radhar, billah_ble_2021, aziz_shah_privacy-preserving_2020, rahaman_tracking_2021, ashleibta_non-invasive_2021, liu_beyond_2019, zeng_multisense_2020, yin_ubiquitous_2022,feng_sitr_2020, gurbuz_american_2021, li_sitsen_2021, yang_rf-eletter_2021, wang_multi-person_2021, fan_-home_2020, saeed_multiple_2022, raeis_human_2021, avrahami_below_2018, liu_wi-psg_2021}. Other works~\cite{zhao2018rf,wang2020uwhear} showed that RF sensors could surpass a visual sensor's capabilities by detecting human posture and activities through a physical wall. More critically, the advent of generative adversarial networks (GANs)~\cite{goodfellow2014generative} has enabled the ability to synthesize images from low-level information, including across modalities~\cite{kezebou2020tr}. Deep learning has enabled us to make privacy-sensitive inferences, as well as creating interpretable data representations from low level structures - both of these capabilities require us to reconsider the privacy perceptions surrounding RF sensors. Thus, we can further simplify \textit{RQ1a} to ask a second question:
\newline 
\textit{\textbf{RQ1b}. What matters more to users when they are forming their privacy perceptions about a device: the data collected by the device (modality and human-interpretability), or the inferences that can be made on that data, or both?}

Theories such as the mere-exposure effect~\cite{bornstein1992stimulus, bornstein2016mere} state that human preference for objects also depends upon their familiarity with those objects. Hence, we also need to explore whether it is possible that a user's perceptions of privacy may be affected by how familiar they are with the device. This sense of familiarity may include whether the user has interacted with that particular device, other devices from the same manufacturer, other devices from the same family of the devices or has worked on those devices in some capacity. This leads us to another question: 
\newline
\textit{\textbf{RQ2}. How does familiarity with a device affect a user's perception of its privacy-sensitivity?}

Human beings create their first-impressions about an object using its physical appearance. This phenomenon is also seen in shopping where the physical appearance of products greatly influences a user's decision to buy them~\cite{creusen2005different}. The physical appearance of an object also invokes a user's familiarity with that object~\cite{bornstein2016mere}. Since sensing devices instrumented in a physical space do not come with any disclosures or labels, users have to rely upon physical appearance to build privacy perceptions of that device. This leads us to our next question:
\newline
\textit{\textbf{RQ3}. How does the physical appearance of a device affect a user's privacy perception of that device?} 
\newline
For example, if a device that is considered to be innocuous, such as a WiFi router, were to look like a more privacy-invasive device, such as a camera, will that affect a user's privacy perceptions?

Finally, with growing user concern over how data is being collected, stored and shared~\cite{wang2016big, wang2016using}, it is important to discuss how the amount of control (or lack thereof) a user has over their data helps shape their privacy perceptions. Recent advancements in machine learning have further exacerbated the rampant unauthorized secondary use of data~\cite{chen2013problematic, oliveira2010privacy}. Furthermore, zero-day vulnerabilities~\cite{bilge2012before} and the constant fear of devices being hacked~\cite{rostami12being} have made users wary of installing sensing devices in their personal space. These implications lead us to our final question:
\newline
\textit{\textbf{RQ4}. How does control over the design of a device and its data policies (type of data collected, its storage and transmission) affect a user's perception of privacy-sensitivity of that device?} 

By answering questions \textit{RQ1b, RQ2, RQ3, RQ4} we investigate user perceptions of privacy surrounding low-dimensional sensor data and how they compare against existing notions of privacy for such data. We use RF sensors such as mmWave radar and WiFi router as examples of low-dimensional sensors for our study due to their ubiquity and a recent surge in their sensing applications. We aim to understand how factors such as modality of sensing (data collected by the device), inferences that can be made on the data, familiarity, physical appearance, and control help shape a user's privacy perceptions regarding sensor privacy.  Intuitively, given that more and more spaces are instrumented with sensors, we aim to validate (or invalidate) prior researchers' notions of privacy given user perceptions. First, we aim to compare the privacy perceptions of data and the inferences that can be made from that data. Second, we study the impact of users' prior knowledge about the properties of the sensor in question, such as the sensor type, form factor, manufacturer, and data-processing algorithm. Finally, we study the perceived privacy impact of a user's control over the device configuration, the data collection, and data storage processes for a given device.

\noindent\textbf{Study Details.} To validate our hypothesis, we performed an online survey study\footnote{exempted as part of IRB approval process} on 162 respondents from the United States to measure users' perception of privacy across the four factors described previously: data information, prior device knowledge, physical appearance and device control. Our study seeks to understand the contribution of each factor in helping shape the privacy perceptions of users. We also present the respondents with scenarios and open-ended questions that allow them to express their thoughts. We then conduct both qualitative and quantitative analysis of the responses to answer our research questions and ascertain the validity of our hypothesis.

\noindent\textbf{Study Results.} The main findings of our study are as follows:
\begin{itemize}
    \item In the case of sensors that collect human-interpretable data (such as cameras), data and inferences can be used interchangeably to inform user decisions regarding privacy.
    \item In the case of sensors that collect non human-interpretable data (such as RF sensors), it is the inferences, rather than data collected, which affects a user's privacy perceptions most.
    \item When the data and inferences are not available, the physical appearance and familiarity of a user with a device type are the primary factors that dictate how users perceive the privacy-sensitivity of a device.
    \item If given complete control over the data policies and device design, users are more likely to instrument their personal spaces with sensing devices. 
\end{itemize}

\noindent\textbf{Research Goals.} Our goal is to study what factors affect the privacy perceptions of a non-expert user when they encounter an IoT device. The factors discussed in this work can be used in conjunction with other conceptions of privacy (\secref{sec:terms}) to better inform future works that aim to instrument user-spaces with sensors.


\noindent\textbf{Contributions.} The main contributions of our paper are summarized as follows:
\begin{itemize}
    \item We rigorously define (\secref{sec:method}) and investigate the factors contributing to a non-expert users' privacy-sensitivity in the context of advances in deep learning for low-dimensional sensor data. To the best of our knowledge, we are the first ones to do so.
    \item We design and conduct a user study that aims to understand the impact of the defined factors that affect a user's privacy perceptions of devices.
    \item We discuss how researchers can utilize our findings to improve their disclosures regarding privacy-sensitivity across sensing applications.
\end{itemize}


==> Sources/2-related_work.tex <==
\section{Related Work}\label{sec:related_work}

We first describe related work on claiming RF to be less privacy sensitive than visual modalities.  We then cover research investigating different dimensions of sensor modalities that affect user privacy perceptions.  Lastly, we cover related research that seek to inform and measure privacy behaviors of sensors and systems. To the best of our knowledge, our privacy study is the first of its kind where we compare data collected from a device to the inferences that can be made on that data in terms of their effects on a user's privacy perceptions. Some other factors that we investigated include:
\begin{itemize}
    \item Physical Appearance: If the user is met with the device, how do they perceive its privacy given its appearance?
    \item Familiarity: How does a user's prior experiences with a device affects their privacy perceptions about the device?
    \item Multiple Types: Are multiple device types (e.g. camera, RF) studied?
    \item Inferences: Does this work investigate different types of inferences and how they affect privacy perceptions?
    \item Modality: Does this work investigate whether privacy depends on the modality of data collection?
    \item Control: Does this work investigate control over device data policies and design, and how they affect privacy?
\end{itemize}




\subsection{Claims without validation: RF is more privacy sensitive than camera/vision}


There is a growing body of work, particularly in the RF domain, which seeks to replace more 'privacy-invasive' modalities (such as cameras) with RF sensing.  The reason for this replacement is at least in part due to concerns of privacy, with some works in this area citing privacy as the primary reason for replacing modalities.  Various application scenarios arise where users may have information they wish to keep private - these scenarios involve sensing and monitoring occupancy in buildings ~\cite{billah_ble_2021, aziz_shah_privacy-preserving_2020}, understanding travel patterns in smart homes ~\cite{gochoo_device-free_2018, rahaman_tracking_2021}, inferring breathing patterns ~\cite{ashleibta_non-invasive_2021, liu_beyond_2019, zeng_multisense_2020, yin_ubiquitous_2022}, detecting posture and gesture at various granularities ~\cite{feng_sitr_2020, gurbuz_american_2021, li_sitsen_2021, yang_rf-eletter_2021, wang_multi-person_2021}, and general daily life and activity monitoring ~\cite{fan_-home_2020, saeed_multiple_2022, raeis_human_2021, avrahami_below_2018, liu_wi-psg_2021}.  However, these works are motivated by a notion of privacy that has yet to be properly understood - a majority of these works directly claim that cameras are more privacy invasive than the RF modality without specifying what this invasiveness means.  In the more extreme cases, some works claim that the RF modality has no issues with privacy at all and is 'non-privacy invasive'.  For several of these works, privacy is the primary reason to choose RF modalities, due to an existing notion of privacy where data is less privacy-invasive if it is less interpretable ~\cite{fan_-home_nodate, raeis_human_2021, avrahami_below_2018}.  

We argue that these claims have not been sufficiently validated, and this notion of privacy itself does not encompass a sufficiently deep understanding of what other modalities are capable of.  Time and time again we witness examples of unexpected privacy-invasive inferences made by various modalities, such as reidentifying users based on accelerometery data ~\cite{saleheen2021wristprint} or sensing sound from RF sensors ~\cite{wang2020uwhear}.  As many of these related works focus on scenarios that monitor a user's daily life and health attributes (which are private from both a personal and legal ~\cite{rights_ocr_summary_2008} perspective), it is imperative that the capabilities of a modality are better understood before such claims are made.  This motivates a need to improve our understanding of what truly makes a sensor 'privacy invasive'.
In our study we seek to correct an existing notion that the privacy perceptions of a particular sensor can be accurately judged based on data interpretability.  Our investigation of existing work has led us to the design of 4 relevant concepts that affect user perception of sensing modalities.  

\subsection{Exploring Privacy Sensitivity of Devices and Sensors}

The 'privacy invasiveness' of a sensor is not solely dependent on the sensing modality.  There are a number of works investigating different dimensions of sensors (appearance, familiarity, etc.) and how they affect perceptions of privacy. \cite{ahmad_tangible_2020} and~\cite{koelle_beyond_2018} explore different physical designs of sensor mechanisms capable of describing sensing state.  More specifically, they explore how certain notifiers and actuators, such as lights and shutter mechanisms, are capable of improving perceptions of privacy. \cite{ahmad_tangible_2020} identifies the concept of 'tangible privacy', which describes a set of physical mechanisms on devices to clearly represent privacy states of IoT devices, with the goal of minimizing uncertainty in certain device states (such as being on or off).  In a similar vein, ~\cite{koelle_beyond_2018} focuses on designs for body-worn cameras that clearly describe their sensing state.  ~\cite{cheng_peekaboo_2019} designs a birdhouse-shaped camera system which grants privacy controls to inhabitants in a home home setting. \cite{leaky_sensor_fields} focuses on redesigning smart home security cameras to both improve adoption while enabling privacy controls. 
In our study, we consider how the concept of physical appearance affects user perception of privacy.  

In addition to physical appearance of sensors, privacy perceptions of sensors are also affected by the setting in which they reside, as well as the manufacturer of those sensors. ~\cite{haney_its_2021}, ~\cite{zheng_user_2018}, and ~\cite{malkin2019privacy} both study perceptions of privacy regarding smart home devices, and how manufacturer trust affect these perceptions.  ~\cite{haney_its_2021} focuses on how users believe responsibility should be assigned when it comes to handling privacy concerns of smart home devices - they consider different combinations of personal, manufacturer, and governmental responsibility.  ~\cite{zheng_user_2018} studies smart home users and their beliefs in privacy protections of devices - they find that both brand familiarity and reputation in device manufacturers plays a primary role in determining trust-based purchasing decisions.  Lastly, ~~\cite{malkin2019privacy} describes trust in different smart speaker manufacturers and how they handle data.   ~\cite{velykoivanenko2021those} investigates the different features of fitness trackers, and how well users understand privacy implications in the fitness-tracker ecosystem.  In this study, we also consider how the concept of manufacturer familiarity and reputation influences privacy perceptions of devices.  

In addition to manufacturer trust affecting privacy perceptions, ~\cite{zheng_user_2018} also studies how data-sharing behaviors from smart home devices is heavily influenced by perceived benefit of sharing.  ~\cite{akter_i_2020} seeks to study image sharing behaviors of visually impaired persons, and how different types of objects present in the images, as well as familiarity with assistants affect sharing decisions.  Unlike these works, we focus on specific data-sharing behaviors when their intended inferences are known.  We choose inferences that have been shown to be possible on both cameras and RF modalities.  ~\cite{jin_exploring_2022} studies smart home privacy-protective behaviors (SH-PPBs), examining how people currently enforce privacy controls over smart devices, as well as raising ideas for new privacy features - such features come in the form of physical design controls, but also as software features (such as a data management portal).  Similarly, our study also aims to understand how varying levels of user control and knowledge of the sensor affects privacy perceptions.  ~\cite{naeini2017privacy} identifies a set of factors influencing privacy preferences in IoT scenarios - in particular, they focus on aspects of data collection of different devices. ~\cite{zeng2017end} explores different levels of familiarity with IoT technologies, and how it influences knowledge of privacy and security risks arising in smart home scenarios.  ~\cite{lee2022understanding} studies different privacy attitudes and privacy concerns regarding data collection via a variety of modalities.  ~\cite{baron2020you} studies the privacy sensitivity of different types of information captured in mobile services.  

In our study of RF and camera modalities, we explore how familiarity, appearance, and inferences from these particular sensors play a major role in privacy perceptions. Unlike previous works, our goal is not to design new sensors, but rather to explore existing sensor designs and consider the different factors affecting user privacy perceptions.  

\subsection{Structuring and Measuring Privacy Properties}


One active area of research relevant to our study is the creation of transparency mechanisms for describing privacy properties of devices and systems.  Creating such mechanisms often requires structuring privacy properties into a set of concepts that are critical to privacy perceptions of users.  Privacy and Security labels ~\cite{emami-naeini_ask_2020} for IoT devices aim to provide concise insight into a device's data collection behavior, enabling consumers to make better device purchasing decisions.  Such methods of improving transparency have already been adopted by companies such as Apple ~\cite{noauthor_privacy_nodate} and Google ~\cite{noauthor_get_2022}, which typically focuses on installation of mobile apps.  In both cases, they distill a set of concepts that are critical to helping users make better privacy decisions.  Concepts include security-update policies, sensor data collection, purpose, manufacturer, and several others.  However, these mechanisms often don't include concepts relating to potential privacy-invasive inferences, such as race, occupancy, and activity recognition.  As we explore different dimensions of privacy-invasiveness in our study, we believe our findings can be complementary to the design of these transparency mechanisms and introduce new concepts.

In addition to creating a structured set of privacy properties that affect privacy perceptions of devices, various works also seek to measure the privacy properties of systems. Some existing methods focus on  mobile applications ~\cite{noauthor_privacygrade_nodate} and websites ~\cite{noauthor_welcome_nodate}. For example, PrivacyGrade ~\cite{noauthor_privacygrade_nodate} aims to assign grades (ranging from A to D) to different mobile applications based on discrepancies in behaviors described by the developer, and the underlying application software. In the web domain, PrivacyScore ~\cite{noauthor_welcome_nodate} seeks to provide a ranking of websites based on presence of a set of security features.  Another broad category of works may also seek to describe formal privacy metrics ~\cite{wagner_technical_2019} from a technical perspective.  Example categories include adversarial success, data similarity, and several others - however, unlike these works, we seek to capture privacy perceptions from a human perspective, with a focus on sensors rather than a system.

Our study is partly inspired by previous works studying various dimensions of sensors.  We structure our study around several critical concepts affecting privacy perceptions in order to break existing notions of privacy-invasiveness for RF sensing.  



==> Sources/3-method.tex <==
\section{Method}\label{sec:method}

In this section, we describe our survey formulation process and data analysis methods.

\subsection{Hypothesis}
In this work, we want to challenge the notion that the most common factor affecting privacy sensitivity of devices is the ability of human beings to understand their data. To evaluate this notion and determine the characteristics affecting privacy perceptions in devices, we came up with a set of 4 factors that affect how a user  perceives the privacy-sensitivity of a device presented to them. In the following sub-sections, we describe these factors and our reasoning behind them.

\subsubsection{Privacy Factor (1): User's Prior Knowledge}
Mere-exposure effect~\cite{bornstein1992stimulus, bornstein2016mere} states that the more familiar~\cite{raghunathan} people are with something, the more preference they have for it~\cite{fang2007examination}. This effect is seen when people stick to the same brand of cars, devices and even engage with same businesses in their daily lives. Building upon this, we want to examine whether user's prior knowledge of a device, family of devices, or the manufacturer plays a role in their privacy perceptions of that device. Specifically, we want to test the following hypothesis: \textit{A user's familiarity with a device and its meta-properties (e.g. manufacturer, device type) affect their privacy perceptions about that device.} 

\subsubsection{Privacy Factor (2): Physical Appearance of the Device}
Human beings tend of build their opinion about objects from the very moment they appear in front of them. Such is the case in shopping where the appearance of products greatly influences a user's decision to buy it or not~\cite{creusen2005different}. Similarly, whether at work or at a public space, when we see a sensor we immediately begin to associate it with what we know.  This association is often on the basis of its physical appearance only, since no other information about that device is available. This physical appearance affects the user's familiarity with said device, which in turn affects privacy perceptions.  At the same time, though the user may be familiar with the device, they may not necessarily be comfortable sharing data from it - one example is a camera, which is familiar but users may not feel comfortable around.  In our study, we want to examine how the physical appearance of a device affects a user's privacy perception of it. Specifically, we want to test the following hypothesis: \textit{If we take a device that users are \textit{comfortable} and \textit{familiar} with, and change its physical appearance to that of a device that they are still \textit{familiar} but \textit{no longer comfortable with}, their privacy perceptions about that device will change to being more negative.} Since familiarity also affects our perception based on physical appearances, this hypothesis is an extension of the previous hypothesis.

\subsubsection{Privacy Factor (3): Interpretable Data Representations}

Several research works in the sensing community~\cite{li2019survey} equate privacy with the ability for a human to make inferences on the raw data collected by that sensor. In~\cite{li2019survey}, the authors claim that RF sensors preserve visual privacy since it does not capture the visual shape of the target - implying that since humans have vision as a sensory modality, devices that collect vision data are more privacy-invasive.  In other words, this notion of privacy is based on using data representations which are less interpretable to humans. Other works describe a similar notion, where RF data is more privacy preserving than visual sensors due to having less-interpretable data representations \cite{fan_-home_nodate, raeis_human_2021, avrahami_below_2018}. However, in a world where the machine learning is used to make inferences of the collected data, this notion is not sufficient to meaningfully ensure privacy. In fact, works such as~\cite{zhao2018rf} show that it is not only possible to extract shape, but also posture of human targets using a radar.


In this study, we want to find out what causes users to perceive a device negatively in terms of it's privacy -- the data representation it collects or the inferences that can be made on that data. More specifically, we want to test the following hypothesis: \textit{When shown the inferences that can be made on the (non-human interpretable) data collected by a sensor, the user's privacy perceptions change about that device}.  Importantly, this allows us to study changes in privacy perceptions when users are made aware of possible inferences from sensor data.


\subsubsection{Privacy Factor (4): Control over Device Design and Data Policies}
As the world moves more and more towards data-driven methods for tasks such as learning user preferences, modeling user behavior and selling ads, users have become wary of what data they share and how it is being used~\cite{wang2016big, hochheiser2015truth, wang2016using}. Often times, even if the data is being used for one purpose, there is no way to tell if the company collecting that data will start using it for another purpose~\cite{brown2004investigating}. Such collected data can be used to make various inferences about users. As a result, we investigate the effects of granting users varying degrees of control over collected data, and how such control affects willingness to adopt sensing devices into their environment.  More specifically, we want to test the following hypothesis: \textit{If given more control over how data is collected, transmitted and stored, users are more likely to instrument their spaces with sensing devices.}


\subsection{Survey Study}

To test our hypothesis we conducted an online survey on the privacy preferences of users from diverse backgrounds. Participants took approximately 12-18 minutes to complete the survey. In the survey, we showed participants images of sensing devices, the data collected by those devices, and the inferences that can be made on that data. In addition, we also posed some situational questions that allowed us to test our hypothesis. In the following subsections, we dive deeper into our survey methodology. 

\subsubsection{Selection of Scenarios}
In our survey, we investigate whether it is the physical appearance, data representation, or the high-level inferences that users most cared about when it came to privacy perceptions. Additionally, we also investigate how familiarity with a sensor or family of sensors affects its privacy perceptions. We followed a three-step approach to decouple various properties from each other. We started by showing users an image of a device and asked them how familiar they are with  said device. Then we asked them to write what they believed the device was. Finally we asked them whether they would be comfortable with installing said device in their bedroom. Since we wanted to keep the study in context with radio-frequency (RF) sensing, we chose to compare user opinions about privacy-sensitivity of cameras with mmWave sensors, WiFi routers, and audio sensors -- all of which are commonly used in sensing tasks. Finally, the respondents were presented with several scenarios that measure perceptions of privacy in the face of varying degrees of control over shared data from a device.



\begin{figure*}[!tbp]
    
        \centering
          \subfloat[]{\includegraphics[width=0.15\textwidth]{SurveyImages/survey_image1-removebg-preview.png}}
          \subfloat[]{\includegraphics[width=0.15\textwidth]{acmart-primary/SurveyImages/Selection_391.png}}
          \subfloat[]{\includegraphics[width=0.15\textwidth]{SurveyImages/survey_image2-removebg-preview.png}}
          \subfloat[]{\includegraphics[width=0.15\textwidth]{acmart-primary/SurveyImages/Selection_393.png}}
          \subfloat[]{\includegraphics[width=0.15\textwidth]{SurveyImages/survey_image3-removebg-preview.png}}
          \subfloat[]{\includegraphics[width=0.15\textwidth]{acmart-primary/SurveyImages/Selection_392.png}}
        
        \caption{We use 3 main classes of devices in our study. Each class has 2 different devices (in order to ascertain that the user responses are dependent on the class of device and not on the device itself.) These devices are \textbf{a)} An Amazon Blink home camera, \textbf{b)} Kasa Inoor Pan/Tilt Smart Security Camera \textbf{c)} A Wayv mmWave radar from Aienstein AI, \textbf{d)} LifeSmart mmWave Human Presence Sensor, \textbf{e)} LinkSys MAX-STREAM AC1300 WiFi router, and \textbf{f)} TP-Link AX1800 WiFi 6 router. In this paper, we use RF devices to learn more about factors that govern user privacy perceptions.}
        \label{fig:survey_devices_methods}
\end{figure*}

\subsubsection{Selection of Devices}
In our survey, we mainly focus on 3 classes of devices -- cameras, RF sensors (such as mmWave radars) and WiFi routers. The goal of our survey is to highlight how users perceive the privacy of RF sensors when compared to cameras (since cameras are considered to be more privacy invasive by existing notions of sensor privacy). For our survey, we selected three devices -- a smart-home camera, a mmWave sensor and a WiFi router. While the WiFi router has become ubiquitous in households, both cameras and mmWave sensors are steadily gaining inroads into the smart-home ecosystem. mmWave based RF sensors have been used for various applications such as human activity recognition~\cite{li2019survey, ding2021radar, singh2019radhar} over the past several years. Similarly, WiFi routers are also being leveraged to make a variety of inferences about users in a space~\cite{wang2017device, li2019wi, chen2018wifi}. Hence, we chose these devices to compare and contrast with a camera. 

To avoid a particular brand name or a form factor affecting a respondent's decision (ascertain that it is the class of device and not the device itself that is being shown that affects a user's response), we select two sets of images for all the three types of devices as shown in \figref{fig:survey_devices_methods}. We presented some respondents with first set of images and other respondents with second set of images. Our results show that both sets of images lead to similar trends in user responses. For cameras and WiFi routers, we select best sellers on Amazon.com while for a mmWave sensor we select commercially available off-the-shelf devices (the choice for mmWave sensors is limited). Our two cameras include an Amazon Blink Mini 1080p camera and a Kasa Indoor Pan/Tilt Smart Security Camera. Both of these are best sellers on Amazon.com. For mmWave devices we selected an indoor mmWave radar called Wayv Air which is manufactured by Ainstein AI and another device called the LifeSmart mmWave Human Presence Sensor. Both of these devices are some of the only commercially available off-the-shelf mmWave devices. For WiFi routers, we choose a TP-Link AX1800 WiFi 6 Router (best seller on Amazon.com) and a Linksys MAX-STREAM AC1300 Dual-Band Mesh WiFi 5 Router. All the six devices are commercially available and can be purchased online. 

\subsubsection{Selection of Sample Data Representations for each Device}
In our survey, we show users a snapshot of the data collected by the sensing devices listed above.  We ask respondents about their privacy comfort levels with a device/sensor being placed in their bedroom. To help them visualize this scenario, we chose a generic camera image of two people sleeping on their bed as this best describes the scenario that our survey mentions. For the mmWave radar, we took a data snapshot from the company's website. Finally, for the WiFi router, we chose the output of Wireshark packet sniffing to show the sample data collected by it. Wireshark~\cite{banerjee2010evaluation} is one of the most popular open-source network analyzer that is widely used to analyze WiFi traffic.

\subsubsection{Selection of Possible Inferences for each Device}

For each sensing device listed above, we showed the respondents a list of potential inferences that can be made on their data. These inferences and the research works that they are derived from are listed below:

\begin{itemize}
    \item \textbf{Camera:} (i) The number of people in the room ~\cite{teixeira2007lightweight}, their clothing~\cite{stearns2018applying, huang2021clothing}, race~\cite{layne2012person}, ethnicity~\cite{layne2012person}, body shape~\cite{guan2009estimating}, height~\cite{guan2009estimating}, and posture~\cite{guan2009estimating}; (ii) Certain activities, behaviors, and health conditions of the people~\cite{ann2014human, demrozi2020human}: having meals, drinking, smoking, walking, praying, watching TV, using a smartphone, intimate moments (hugging, kissing), and breathing rate~\cite{massaroni2018contactless}.
    \item \textbf{mmWave Radar:} (i) The number of people in the room ~\cite{choi2017people, weiss2020improved}, body shape, height, and posture~\cite{li2020capturing, sengupta2020mm}; (ii) Certain activities, behaviors, and health conditions of the people~\cite{li2019survey, ding2021radar, singh2019radhar}: having meals, drinking, smoking, walking, praying, watching TV, using a smartphone, intimate moments (hugging, kissing), and breathing rate~\cite{wang2020remote, chauhan2020through}.
    \item \textbf{WiFi Router:} (i) Websites that have been visited, total time spent on a smartphone, and sleep schedule~\cite{ohm2009rise, hernandez2021reduction}; (ii) The number of people in the room ~\cite{yang2018wi, cheng2017device}, body shape, height, and posture~\cite{jiang2020towards, ren2022gopose}; (iii) Certain activities, behaviors, and health conditions of the people~\cite{wang2017device, li2019wi, chen2018wifi}: having meals, walking, praying, watching TV, using a smartphone, intimate moments (hugging, kissing), and breathing rate~\cite{abdelnasser2015ubibreathe, gao2020device}.
\end{itemize}

\subsubsection{Measuring Privacy Perceptions}\label{sec:data_inferences_privacy}
To gauge how concerned users were regarding the privacy aspects of a sensor, we asked them the following questions:

\textit{\textbf{Q1}. How comfortable are you with this device being placed in your bedroom and streaming/recording data? (an image of the device is shown to the respondents)} We start out with this question since the the form factor of the device and its appearance are the first things that users notice. Even before they are able to read more about the device, examine the data it collects or look at the inferences that it makes, they are already forming privacy perceptions of a device. 

\textit{\textbf{Q2}. The data collected by the device shown below looks like the image on the right. How comfortable are you with this device being placed in your bedroom given the data that it collects? (an image of the device and the representation of its collected data is shown to the respondents)} This question helps us measure how much the human ability to interpret data plays into the notions behind privacy. This also helps us evaluate the claims about privacy made by research works that use the human ability to understand raw data as a measure of privacy.

\textit{\textbf{Q3}. The device shown below is from a company that promises that no humans look at the raw sensor data captured by these devices - instead, only specific information (as a result of processing) is shared. The processing algorithms can make the following inferences about your activities, behaviors, and surroundings:  [List of inferences]. How comfortable are you with such a device being placed in your bedroom and sharing the inferences shown above? (an image of the device is shown to the respondents)} In this question, we explicitly tell the respondents that the data collected by the devices are not shared with any human beings - instead, only the inferences, as a result of processing, are shared. This helps us decouple the notion of data representations from inferences and to see which of the two matters more to the user in terms of privacy notions.

\subsubsection{Equating Privacy Sensitivity with Comfort}
\textit{Privacy-sensitivity} and \textit{privacy-invasiveness} are vaguely defined terms for describing privacy perceptions, and it is difficult to convey their meaning to a non-technical user. Existing research works that aim to measure privacy perceptions use questions like \textit{how comfortable?} to understand a user's privacy expectations~\cite{akter_i_2020}. In our survey, we also use this as a proxy for understanding privacy perceptions. The respondents answers to subjective questions in our survey show that our question formation was able to convey the meaning properly to them.

% \subsubsection{Response Scale}
During the survey, the respondents were able to respond to questions on a 5-point Likert scale~\cite{joshi2015likert}. For familiarity, the scale was: (1) Very unfamiliar, (2) Unfamiliar, (3) Have some idea, (4) Familiar, and (5) Very familiar. For comfort, the scale was: (1) Very uncomfortable, (2) Uncomfortable, (3) Neutral - Neither comfortable nor uncomfortable, (4) Comfortable, and (5) Very comfortable.

\subsection{Choosing a Common Private Space}
In the US, a house is considered a private space~\cite{lawinsider}. Out of all parts of this private space, bedrooms are considered to be the most private~\cite{berry_2020}. People use various parts of their homes in different ways and may not always have a high expectation of privacy there. Such is the case in home rentals where the host may place cameras and other sensors in common areas of the house.  However, instrumenting spaces like bedrooms with sensors (such as cameras) is not allowed. Since people consider their bedrooms to be a sacred and private space~\cite{berry_2020}, we used the scenario of bedrooms as a tool to help us learn about a user's privacy perceptions. 

\subsection{Organization of the Survey}
The survey contains 51 single-choice and subjective (open-ended) questions. The entire survey is available in the appendix. The survey was organized as follow:
\begin{itemize}
    \item Consent form that describes who is collecting the data, why is it being collected and how it will be shared with other researchers.
    \item Demographic questions about age, gender, annual income, educational background, and familiarity with technology to learn how these factors play into privacy perceptions.
    \item We show users an image of a device, ask them what they think it is,  how familiar they are with it. Then we ask them how comfortable they are if said device is installed in their bedrooms.
    \item In the next section, we show the users an image of a device and a snapshot of the data that it collects.  We then ask them how comfortable they are if said device is installed in their bedrooms.
    \item In the next section, we show users images of various devices, and a set of inferences that can be made on the data collected by the device. We also describe a scneario where the manufacturer of the device has promised not to share the raw data with any human, and only share certain inferences. We ask the users again about how comfortable they are if said device is installed in their bedrooms.
    \item We present the users with a hypothetical scenario in which we ask them to assume that they create their own camera from scratch and then ask them how comfortable they are if this camera is installed in their bedrooms.
\end{itemize}

\subsection{Data Analysis}
In this section, we describe our data analysis procedures, both quantitative and qualitative.

\subsubsection{Quantitative Analysis}
The data collected in the survey does not meet the assumptions of parametric tests -- normal distribution and equal variance of errors. This is because the users have responded with extreme opinions (very uncomfortable or very comfortable) for several questions in the survey. We have one dependent variable -- comfort level and several independent variables (physical appearance, data, inference, control, and familiarity).

To analyze our data, we choose non-parametric tests such as the Wilcoxon signed-rank test, \kstest and the Spearman correlation coefficient test with associated p-value. We use the Wilcoxon test because our study has a repeated-measure design. When having such a design, there might be dependencies among participants' responses to these repeated questions. hence we use the Wilcoxon signed-rank test which is a repeated measures test of dependency. It is performed between two paired groups and used to measure the whether the two related paired samples come from the same distribution. The null hypothesis for the Wilcoxon signed-rank test is \textit{that two related paired samples come from the same distribution}. The \kstest is used to find similarity between two distributions. The null hypothesis of \kstest is \textit{that the two distributions are similar}. Additionally, the statistic $D$ of the \kstest is small (closer to 0) when the two distributions are similar and close to 1 when the two distributions are different. Suppose we have two distributions $F$ and $G$.  The Spearman correlation coefficient test with associated p-value is used to measure monotonicity of the relationship between two datasets. The p-value indicates \textit{the probability of an uncorrelated system producing datasets that have a Spearman correlation at least as extreme as the one computed from these datasets.\footnote{The definitions of the tests have been taken from their respective pages in the Scipy documentation.}} 

In addition, we also use the mean $\mu$, standard deviation $\sigma$ and $95\%$ confidence interval to describe the overall distribution of user opinions. The user opinions can range from a value of $1$ to $5$ where $1$ means are very negative opinion and $5$ means a very positive opinion. 

\subsubsection{Qualitative Analysis}
The survey contains several questions where respondents were allowed to give open-ended answers. For each device shown to the respondents, we asked them to name what they think the device was. Additionally, we also asked the users two scenario based open-ended questions. These questions were:
\begin{itemize}
    \item \textit{OE1. Suppose you create your own camera from scratch. You control what the camera looks like, what parts go inside it, what data it collects, and where the data is stored. How comfortable would you be with that camera being placed in your bedroom given that no one else can see the data except you? Please explain the choice you made in the previous question briefly.}
    \item \textit{OE2. Which of the following cameras will you prefer if you have to place one inside your home? [The choices were: (i) A camera from a well-known brand that does not sell ads or ad revenue is not a major revenue source for them, (ii) A camera from a company whose main source of income is ad revenue and sells your data to advertisers, (iii) A camera from a company based in the USA, (iv) A camera from a company based in a country that you do not trust]Please explain your answer in the previous question briefly.}
\end{itemize}

In order to better understand how a user's privacy perceptions change when give more control over the data policies and the design of the device, we perform qualitative analysis on \textit{OE1}. All the open-ended answers were coded in a bottom-up approach using inductive coding by two researchers. The researchers met frequently to discuss and iteratively code the answers. The agreement between the researchers was measured using Cohen's Kappa (threshold = $0.8$).


\subsection{Recruitment}

We conducted our survey on Prolific~\cite{palan2018prolific} [Now prolific.co] during June and July 2022. During the survey, we set a filter to only allow respondents in the US and 18 years or older to participate in the survey. The respondent matching was done by Prolific. Each user was able to participate in the survey once. 

\subsection{Compensation and Ethical Considerations}

We recruited the participants through Prolific. The participants were free to choose to participate in the survey. Once the participants selected the survey, they were redirected to a Google form where they were shown a consent form describing the purpose of the study, as well as how the data will be collected and stored. After reading the consent form, the participants could back out of the survey if they chose to do so, without any penalty. After completing the survey, the participants downloaded a `completion code' and entered it into their Prolific account to mark themselves as complete. Each participant was paid $\$2.75$ for completing the survey. Based on the time taken by each respondent, that amounted to a rate of around $\$16.75$/hour (based on calculations done by Prolific). The study was exempted by our institutions review board (IRB) as a part of the IRB approval process.

\subsection{Data Release}
The responses collected during the survey have been anonymized (the Prolific ID associated with each response has been deleted) and the responses are available publicly at: Link Hidden for Anonymity Purposes.


==> Sources/4-Findings_quant_gpt.tex <==
\section{Findings: Quantitative Analysis}\label{sec:quant_find}

\subsection{Demographics}
Of the 162 survey respondents, 58\% were male, 39.5\% female, 1.85\% non-binary, and 1 identified undisclosed. Age-wise, 3.1\% were under 20, 67.9\% between 21 and 40, 24.1\% between 41 and 60, and 4.9\% over 60.

\subsection{Education and Technical Familiarity}
Regarding education, 32.1\% reached high-school, 14.2\% Associates, 31.5\% Bachelors, 19.8\% Graduate, and 2.5\% Professional. Based on a modified Mozilla survey, 10.5\% self-identified as tech experts, 58\% as savvy, 29.6\% as average, and 1.9\% as novices.

\subsection{Privacy Perceptions: Data vs Inferences}
We examined users' comfort levels regarding device placement in bedrooms based on device visuals, data representations, and potential inferences (see \figref{fig:survey_devices_methods}).

\subsubsection{Camera}
Most users (124/162) were uncomfortable with a camera in their bedroom after seeing its image. Revealing its captured data increased this number to 141. Contrastingly, when shown potential inferences, 137 found it intrusive. Both data and inferences led to comparable privacy concerns for cameras.

\begin{figure}[h]
\centering
\includegraphics[width=0.96\linewidth]{acmart-primary/Figures/camera_likert.pdf}
\caption{Comfort levels with a camera based on (a) its image, (b) captured data, (c) potential inferences.}
\label{fig:camera_responses}
\end{figure}

\subsubsection{mmWave Radar}
For the less familiar mmWave radar, 88/162 felt uneasy with it in their bedroom based on its image. This dropped to 71 after seeing its non-human interpretable data but rose to 117 when exposed to the inferences, reflecting a significant difference in user perception between raw data and its implications.

\begin{figure}[h]
\centering
\includegraphics[width=0.96\linewidth]{acmart-primary/Figures/radar_likert.pdf}
\caption{Comfort levels with mmWave radar based on (a) its image, (b) captured data, (c) potential inferences.}
\label{fig:radar_responses}
\end{figure}


==> Sources/5-Findings-qualitative.tex <==
\section{Findings: Qualitative Analysis}\label{sec:qual_find}

In this section, we analyze and group users' subjective responses to the following question in our survey, in order to better understand the factors that guide a user's privacy decision making process:

\noident\textit{OE1. Suppose you create your own camera from scratch. You control what the camera looks like, what parts go inside it, what data it collects, and where the data is stored. How comfortable would you be with that camera being placed in your bedroom given that no one else can see the data except you? Please explain the choice you made in the previous question briefly.}

We first categorized the sentiment of user responses as either positive or negative -- positive if their response suggested that they were comfortable with the camera being placed in their bedroom and negative is they were not comfortable with the camera being placed in their bedroom. The sentiment was analyzed by the two researchers coding the qualitative responses using the open-ended answers. 

\begin{figure}[h]
\centering
\includegraphics[width=0.96\linewidth]{acmart-primary/Figures/qual_analysis_neg.pdf}
\caption{We employed inductive coding to code the open-ended responses. For the answers with a negative sentiment, the following themes (in blue) and codes (in red) emerged.}
\label{fig:code_neg}
\end{figure}

\subsection{Why users don't want to place a camera in their bedroom even when given complete control over it's design and data policies?}

From the responses with a negative sentiment, our inductive qualitative analysis method yielded ten codes. These codes can further be organized into three distinct themes. \figref{fig:code_neg} shows these codes (red) and their associated themes (blue). We describe each theme in more detail below.

\subsubsection{The Fear of Unauthorized Data Access}
In our study, 43 (26.5\%) out of the total 162 respondents expressed some concern regarding their data being accessed without their authorization. Not only is this the case when companies are storing their data but also for devices that they design and control themselves. This unauthorized access can include data breach (N=21), device being hacked (N=24), lack of a user's expertise with designing security focused device (N=3) and other security risks that modern internet-connected devices face (N=1)\footnote{multiple codes can be assigned to the same response.}. One respondent mentions: \textit{All systems are hackable. I will never be ``the only person" who has access to any digital input/output. Privacy does not exist in this world.} Other users said: \textit{``Cameras are hacked all the time. If someone wants it, they will get it. If I made it myself I would be even more wary"}, \textit{``Even though I know that no one else can see the data, I would irrationally believe that somebody eventually would see the data. So I would continue to be uncomfortable with the camera."}, and \textit{``There is never a guarantee that no one else can see the data but me, that's a wishful fantasy, but if data exists its unlikely to stay with only one person"}. One user mentioned \textit{``There's no such thing as a completely secure piece of technology if it can connect to the internet at all."}. This shows the despite given complete control over the design of the device and its data policies, some users still believe that their data can be accessed by others. In fact, some users are more concerned about privacy if they had created a device, since a manufacturer will be able to do a better job than them when it comes to protecting the data and implementing state-of-the-art security techniques. 

\subsubsection{Uneasiness with Sensing}
Despite knowing about the inferences or given full control over the device some respondents were not comfortable with instrumenting their bedrooms with a camera. 30 (18.5\%) out of the total 162 respondents were concerned with a sensor such as camera being placed in their bedrooms as they either found it ``weird" or as something that will cause them paranoia. This uneasiness with sensing can be caused by a fear of being recorded (N=10), a perceived violation of personal space (N=8), a perceived violation of privacy (N=2), not wanting a camera for unspecified reasons (N=9), and a lack of device knowledge (N=2). Several respondents made comments such as: \textit{``I would still feel as if I'm being watched", ``I don't want a camera in my bedroom at all", ``I don't want a camera in my bedroom even if no one else could see it"}, \textit{``It would still feel like there is something watching me at all times..."}, \textit{``I don't like cameras in my bedroom it creates the wrong atmosphere and makes me uncomfortable knowing something is always recording"}, \textit{``all this stuff is like spying to me", ``...a camera in general makes me feel like I'm on display"} and \textit{``Even though no one else can access the data, I still feel uncomfortable having everything filmed in my bedroom.  I don’t want to record my every movement and activity, even if no one else can view it."} This shows that despite the best intentions of a manufacturer, there are users who don't want their private spaces monitored. One needs to be mindful of such preferences when instrumenting spaces with sensors and devices.

\subsubsection{Lack of a Use Case}
In addition to above specified themes, we also found out that 3 ($1.85\%$) users did not want to install any cameras in their bedroom as it served no purpose to them. These users wrote \textit{``This type of camera does not serve a purpose to me", ``..I do not have a necessity..", and ``...I also have no reason to put a camera in my room."} This shows that manufacturers should try to prove the utility of their devices to the users. Instrumenting a space with sensing devices without consulting the users about their needs and doing a use-case study should be avoided.


\begin{figure}[h]
\centering
\includegraphics[width=0.96\linewidth]{acmart-primary/Figures/qual_analysis_pos.pdf}
\caption{We employed inductive coding to code the open-ended responses. For the answers with a positive sentiment, the following themes (in blue) and codes (in red) emerged.}
\label{fig:code_pos}
\end{figure}

\subsection{Why users are likely to place a camera in their bedroom even when given complete control over it's design and data policies?}

In addition to analyzing why users don't want to instrument their personal spaces with a camera, we also analyzed the positive responses -- reasons why users wanted to instrument their spaces with cameras. Our inductive qualitative analysis method yielded five codes. These codes can further be organized into three distinct themes. \figref{fig:code_pos} shows these codes (red) and their associated themes (blue). We describe each theme in more detail below.

\subsubsection{Utility}
Some users are likely to instrument their spaces with cameras is due to the utility that is provides. In our survey, respondents stated \textit{``If I lived with other people I might want to know if other people are going in my bedroom "} and \textit{``i would let it only collect data if there was a break in"}. This shows that demonstrating utility is a possible method that can be used to improve the adoption rate of a particular device.

\subsubsection{Control over the device}
By far, a majority of users wanted to place a camera in their bedroom largely because they can control its data collection (N=19) and the access to collected data (N=40). Several respondents noted \textit{``I control what it sees so it doesn't worry me", ``If I could control what it saw and collected I might be ok with it", ``If I can control the flow of data, I am comfortable with placing the device in my bedroom", ``If I had complete autonomy of what the data collects and how it is used, and I only have access to it, I would feel very comfortable because I would design it to suit my privacy needs and protect myself"}, and \textit{``There is no chance that my personal data could be used in the wrong way if I have total control of how it’s used."} These comments validate our hypothesis that a user's notions about the privacy sensitivity of a device depend upon the amount of control they have over it.

\subsubsection{Knowledge of the device}
Additionally, we also find that the more knowledge about how a device works that users have, the more likely they are to use it appropriately. In our survey, several (N=11) users said that since they knew how the device works, they are fine with placing it in their bedrooms. Some responses included \textit{``If I know what it is doing at all times I wouldn't mind it being in my room", ``I would know exactly what is collected and where the data is going"}, and \textit{``Now that I know what it’s used for, I’m not worried about other companies collecting my data"}.

==> Sources/6-Discussion.tex <==
\section{Discussion}\label{sec:dicussion}

In this section, we discuss key findings of our work, how they can be used by the general community and some limitations of our study.

\subsection{Key Findings}
Our results show that perceptions of privacy do not solely depend upon the intepretability a sensor's data representations, but also on other factors such as possible inferences, physical appearance, familiarity and control. Our main findings are summarized below:

\noindent\textbf{Data Representation vs Inference:} When the data collected by the sensor is human interpretable, it does not matter which of the two are shown to the users as users can make inferences themselves by looking at the data. However, when data is not human intrepretable, we found that inferences have more affect on the overall privacy perceptions of the user. In case of both mmWave radar and WiFi router, showing inferences caused a larger negative shift in the overall privacy perception of the device than the data.

\noindent\textbf{Physical Appearance and Familiarity:} We found that users were less likely to install sensors in their homes that they are not familiar with. Additionally, when users look at a device, they try to find associations between the appearance of that device and any other device that they may have come across. This is evident when users see a router that looks like a camera and mistake it to be a camera and hence change their perception completely. When data and inferences are not disclosed, people use physical appearance and their sense of familiarity to make any judgements about the device.

\noindent\textbf{Control:} When given full control over the device design and data policies, users are more likely to install sensing devices in their private spaces and have an improved privacy perception of the device.


\subsection{Limitations of our Study}

This section discusses some limitations in our study that future research can address. In this study, we showed the users images of a sensor, the data collected, and a list of inferences that can be abstracted from the data. A more thorough in-person study can collect user data using a variety of sensors and show the collected data and the inferences to the users and then ask them about their privacy perception. We expect that when users see their own data and inferences instead of someone else's, it may have a higher impact on their opinions. This approach is analogous to ex-post transparency studies that visualize users' personal data disclosure~\cite{murmann2017tools}. Moreover, future work can contextualize the inferences from sensor data in current data-sharing practices in commodity markets, e.g., understanding how user opinions change before and after they learn how companies might share these inferences with third parties~\cite{farke2021privacy}. Finally, our study only focuses on sensors in spaces with a high expectation of privacy, such as bedrooms. Future studies can also learn how users' privacy expectations change with the space where the sensors are present (e.g., bedroom vs. balcony).

%\subsection{Implications: How Can the IoT/Sensing Community use this Study?}
\subsection{Rethinking Privacy in Future IoT/Sensing Privacy Research}

In this section, we discuss how researchers, manufacturers and users can use the implications of our study to guide future research, design, and instrumentation of sensing spaces.

\noindent\textbf{Avoiding Assumptions about Sensor Privacy.} In light of this study, we hope researchers will avoid using blanket statements about the privacy-sensitivity or privacy-invasiveness of devices such as RF sensors, without a user study. Users are key stakeholders in deciding the privacy viability of sensors and sensing paradigms, and they should have a say in what gets instrumented in their spaces.

%\subsubsection{Future Directions in IoT Privacy Research}
%In light of the findings in this paper, we believe that now is the time to fundamentally rethink how researchers approach the idea of privacy and privacy policies. Relying solely upon human interpretability of sensor data as a predictor for privacy-sensitivity of a device is misguided. We believe that laws and policies need to account for the recent advancements in machine learning in order to determine what type of data to collect from human subjects. Our recommendations are not just useful for RF sensors but can also be applied to any sensing modality. We further describe our recommendations below.

\noindent\textbf{Sensor Privacy in the ML world:} Relying solely upon human interpretability of sensor data as a predictor for privacy-sensitivity of a device is misguided. We believe that laws and policies need to account for the recent advancements in machine learning in order to determine what type of data to collect from human subjects. Our recommendations are not just useful for RF sensors but can also be applied to any sensing modality. 

Today, machine learning algorithms are used in all facets of our lives for various decision making tasks. In future research, instead of only asking \textit{What inferences can a human make from this data?}, we need to ask \textit{What inferences can a machine learning model abstract from this data?} Recent advances in visual-language intelligence that can convert one modality to another such as DALL-E~\cite{ramesh2021zero} show that it is now possible to transform text to images. Since our study highlighted the impact of inferences from RF sensor data on user privacy notions, future researchers can extrapolate to scenarios where the embeddings in sensor data-based machine learning models will increasingly carry more semantic information that, in theory, can also be translated to imaging data understandable to humans. Thus, future research can understand the semantic information encoded by sensor data, which may enable future privacy-preserving techniques, e.g., as is done with privacy-preserving techniques for visual images~\cite{kawamura2020privacy}. %\textit{w from converting these inferences back to images using DALL-E?} Hence,  ML-driven inferences need to be treated as the a key factor in understanding privacy preferences.

\noindent\textbf{Sensor Privacy Disclosure.} There have been several attempts such as the nutrition label for privacy~\cite{kelley2010standardizing} that aim to disclose information about what the sensor is, what type of data does it collect, why is the data being collected, or where the data is stored. When implemented, such approaches can help users learn more about a device and make a better decision about their comfort and privacy expectations with installing such a device in their spaces. However, in light of the key findings in our paper, we believe that every manufacturer should also disclose three more things about a device to better guide this decision making process -- (1) inferences that will be made on the data (2) inferences that can possibly be made on the data collected and (3) an example of some common devices and sensors that are similar to the device in question in terms of functionality. The manufacturers can collect a list of all possible inferences that can be made on the data collected by the sensor from research papers and then divide them into simpler categories. For example, radar sensors can: understand the shape and size of the scene, shape and size of objects and human subjects in the scene, activities being performed, gestures being made, speed of objects, vibrations in the surfaces (which can be used to recreate sound) and vital signs. Disclosures that focus on inferences and use easy to comprehend language for non-technical users need to be used in spaces where privacy needs to be prioritized. 

\noindent\textbf{Sensor Privacy Control:} In order to make users feel more comfortable, device manufacturers and researchers can work together to create paradigms where users have more control over the design and placement of the device without sacrificing utility. In addition, data policies need to allow users the right to have their data deleted when they want to. Before using the data for training new models or for selling ads, express user consent needs to be sought. Finally, in some cases, control means the right to not be monitored at all. The idea that some users wish to remain anonymous and out of range of any sensing device needs to be respected as well.






